Heterogeneous Federated Learning Using Knowledge Codistillation

Federated Averaging, and many federated learning algorithm variants which build upon it, have a limitation: all clients must share the same model architecture. This results in unused modeling capacity on many clients, which limits model performance. To address this issue, we propose a method that involves training a small model on the entire pool and a larger model on a subset of clients with higher capacity. The models exchange information bidirectionally via knowledge distillation, utilizing an unlabeled dataset on a server without sharing parameters. We present two variants of our method, which improve upon federated averaging on image classification and language modeling tasks. We show this technique can be useful even if only out-of-domain or limited in-domain distillation data is available. Additionally, the bi-directional knowledge distillation allows for domain transfer between the models when different pool populations introduce domain shift.

==> 3_related_work.tex <==
\section{Related Work}\label{app:related_work}


%\textcolor{red}{TODO}
\citet{mora2022knowledge} present an overview of Knowledge Distillation (KD) techniques for Federated Learning (FL). In one set of approaches, client models transfer knowledge to a centralized served model~\citep{seo2022}, In the second set, called \emph{co-distillation}~\citep{anil2018}, an ensemble of clients learn without a central server model. \citet{jeong2018communication} propose a distillation strategy that significantly reduces communication costs by exchanging soft targets instead of model parameters between the server and clients. In this approach, the clients transmit their per-label averaged logits computed on their private data, and the server averages these logits and broadcasts them in the next round. The clients then regularize their local loss using the server's logits. Variants of this method are presented by \citet{oh2020distill, ahn2019wireless, ahn2020cooperative}. \citet{itahara2020distillation} demonstrate that this technique does not perform as well as \fedavg\ on non-IID data in terms of communication cost and accuracy. They present a variation where clients compute logits on unlabeled data, which are then averaged to compute a global logit after applying a temperature parameter that is chosen to minimize the entropy of the softmax. Their strategy leads to a lower communication cost and better accuracy than \fedavg.

\citet{lin2020} investigate the use of ensemble distillation in FL, which solicits logits rather than parameters from federated clients. In this method, the server computes an ensemble based on the logits from the client models, and then uses these logits to update a set of models for each architecture group, thus allowing information to be shared across all groups. 
%This approach achieves a significant speed-up in convergence compared to FedAvg and other FL techniques. 
Our approach also relaxes this assumption by dividing the clients into pools based on capacity and training a model within each pool using \fedavg. While \citet{lin2020} diverge from \fedavg\ in using client logits for constructing server models, we use \fedavg\ as a building block. We propose two alternative strategies for co-distillation, which enables the client pools to learn from each other. Thus it is different from the method in \citet{lin2020} that uses all clients, regardless of capacity, to update server models of different architectures/sizes. One potential advantage of our approach is that clients within a pool typically have similar characteristics, which will likely reduce entropy of output distributions in each pool. \citet{afonin2021towards} present a theoretical framework for KD in FL, showing that the performance is limited by data heterogeneity. \citet{ozkara2021quped} propose a KD approach for learning personalized FL models where the clients can differ in terms of architecture and weight precision.

==> 4_experiment_setup.tex <==

\newpage
\section{Experiment Setup}\label{app:setup}

\begin{table*}[h]
\caption{Dataset sizes used for the experiments. The distillation datasets for federated CIFAR-100 and StackOverflow are excised from the original datasets' training split, as is the held-out set for CIFAR-100. StackOverflow has default held-out and test sets of $\sim$16M examples each. From each, we draw 5,000 and 100,000 examples for tuning and evaluation, respectively.}
\label{tab:data}
% \vskip 0.15in
\vspace{-0.1cm}
\begin{center}
\begin{small}
\begin{sc}
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{l|c|cc|c|r}
\toprule
\multirow{3}{0em}{Dataset}  & Distillation & \multicolumn{2}{ c }{Federated Pool} & \multicolumn{1}{| c }{Held Out}& \multicolumn{1}{| r }{Test} \\
& Examples & Clients & Examples & Examples & Examples \\
\midrule
CIFAR-100   & 13,500  & 315  & 31,500  & 5,000  & 10,000 \\
CIFAR-10    & 50,000   &   &  &  \\
\midrule
% StackOverflow    & & 342,477 & 135,818,730 & 38,758 & 16,491,230 & 204,088 & 16,586,035 \\
StackOverflow    & 122,250,952  & 34,248 & 13,567,778 & 100,000 & 100,000 \\
C4-mod    &  4,488,694 &   &  & &  \\
% \multirow{3}{0em}{Dataset}  & Distillation & \multicolumn{2}{ c }{Federated Pool} & \multicolumn{2}{| c }{Held Out}& \multicolumn{2}{| c }{Test} \\
% & Examples & Clients & Examples & Clients & Examples & Clients & Examples \\
% \midrule
% CIFAR-100   & 13,500  & 315  & 31,500 & 50  & 5,000 & 100 & 10,000 \\
% CIFAR-10    & 50,000   &   &  &  &  &  &  \\
% \midrule
% % StackOverflow    & & 342,477 & 135,818,730 & 38,758 & 16,491,230 & 204,088 & 16,586,035 \\
% StackOverflow    & 122,250,952  & 34,248 & 13,567,778 & 38,758 & 16,491,230 & 204,088 & 16,586,035 \\
% C4-mod    &  4,488,694 &   &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
\end{sc}
\end{small}
\end{center}
\vskip -0.15in
\end{table*}

To evaluate \inter\ and \merged, we run experiments on the tasks of image classification and language modeling, comparing against a baseline of \fedavg. For image classification experiments, we use the federated version of the CIFAR-100 dataset\footnote{\tiny \url{https://www.tensorflow.org/federated/api_docs/python/tff/simulation/datasets/cifar100}} \cite{krizhevsky2009learning}, supplemented by CIFAR-10 as out-of-domain distillation data. For language modeling, we use federated Stack Overflow (SO)\footnote{\tiny{\url{https://www.tensorflow.org/federated/api_docs/python/tff/simulation/datasets/stackoverflow}}}, which we supplement with out-of-domain distillation data drawn from the C4 \cite{raffel2020exploring} dataset and modified to match the casing and tokenization of the SO data; we refer to this as C4-MOD. All dataset sizes are shown in Table~\ref{tab:data}. For both CIFAR-100 and SO datasets, we hold out 10\% of the original train split as validation data.

All experiments are run in the FedJax framework~\cite{fedjax}, and all hyper-parameters are tuned on the held-out sets through the Vizier hyper-parameter tuning service\footnote{\tiny \url{ https://cloud.google.com/ai-platform/optimizer/docs/overview}} \cite{golovin2017google} with default settings, to a max of 1024 trials.\footnote{Details of hyper-parameter tuning are shown in Appendix~\ref{app:tuning}.} As all experiment runs have both `small' (low-capacity) and `large' (high-capacity) server models, we tune hyper-parameters to maximize the average accuracy of the two models on the held-out set.


\begin{table*}[h!]
\vspace{-0.2cm}
\caption{\label{tab:data_equal}Data splits for the initial set of experiments.}
% \vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\resizebox{1.0\columnwidth}{!}{%
\begin{tabular}{c|c|cc|cc}
\toprule

 & distillation data & \multicolumn{4}{c}{federated pools}\\ % & \multicolumn{2}{|c}{SO} \\
 &  & \multicolumn{2}{c|}{full pool ($\pool$)} & \multicolumn{2}{c}{high-capacity ($\mainpool$)}  \\%& small & large \\
 & examples & clients & examples & clients & examples \\%& small & large \\
\midrule
CIFAR & 13,500  & 315 & 31,500 & 47 & 4700 \\%& 26.29 & 26.82  \\
StackOverflow  & 122,250,952  & 34,248 & 13,567,778 & 684 & 296,597 \\%& 26.1 & 26.62  \\
\bottomrule
\end{tabular}
}

\end{sc}
\end{small}
\end{center}
\vspace{-0.3cm}
\end{table*}



\subsection{Image Classification}
For the CIFAR-10 and CIFAR-100 datasets, we pre-process all examples with the default settings in FedJAX; all images are centered and normalized, and training images are randomly cropped and horizontally flipped. When using the data for distillation, we apply additional random flipping, which may be vertical or horizontal, and mixup~\cite{mixup} with $\beta=2$. 

For all image classification experiments, we train Convolutional Neural Network (CNNs)~\citep{goodfellow2016deep} with five layers; for the model trained on the high-capacity pool, hereon the `large' model, we train with approx 410k parameters. For the model trained on the low-capacity pool, hereon the `small' model, we train with approx 109k parameters. The details of the model architectures are given in Appendix~\ref{app:model_architectures}.

\subsection{Language Modeling}
For the StackOverflow dataset, we tokenize with a lower-cased 4k word-piece model~\citep{wordpieces}\ fit to the training split. To render the C4 data in the same format as the SO data, we pre-process the C4 dataset by lower-casing and word-tokenizing the first sentence from each C4 example paragraph.\footnote{Word and sentence tokenization via NLTK \cite{bird2009natural}} We additionally correct the remaining differences to the SO tokenization by replacing a small hand-coded list of incorrectly tokenized contractions.\footnote{This list is shown in Appendix~\ref{appendix:contractions}} As the full C4 dataset is substantially larger than what we require for distillation data, we draw from it a subset of 4.5M examples. We train LSTMs~\cite{lstm} with one layer for the `small' model and two layers for the `large' model. 
For the `large' model, we train with approx 4.3M parameters and the `small' with approx 2M parameters. The details of the model architectures are given in Appendix \ref{app:model_architectures}.

For the language modeling runs, rather than using the entire default held-out and test sets with $\sim$16M examples, we draw 100k examples from each. We tune hyperparameters on the held-out set and report accuracy on the test set. To simulate a practical federated learning setting that is constrained in both modeling capacity and data availability, in all experiments, we use only a subset of the federated training pool of the StackOverflow dataset, leaving the remainder of examples unused, or for use as in-domain distillation data.

\subsection{Federated Averaging Baseline}
For all experiments, we use a set of shared \fedavg\ settings. All experiments are run for 1500 federated rounds, sampling 20 clients per round. The clients are optimized with SGD with a constant learning rate. We set the client batch size to 20; all clients train locally for one epoch. We optimize the server models with FedAdam \cite{kingma2014adam,reddi2020adaptive}, using the default hyper-parameters,\footnote{$\beta_1=$\,\,0.9, $\beta_2=\,\,$0.999, $\epsilon=$\,\,1e-5} and with separate tuned learning rates for the large and small models.  We use a linearly decaying learning rate (with a zero final value) over the course of the federated rounds.

\subsection{Distillation}

For each teacher model, we tune a softmax temperature parameter $T > 0$
which may either sharpen (when $T < 1$) or smooth (when $T > 1$) the output probability distribution: $p(y_i) = \frac{\exp\left(\frac{z_i}{T}\right)}{\sum_{j} \exp\left(\frac{z_j}{T}\right)}$, where $y_i$ is a label and $z_i$ is the corresponding logit. We additionally tune a student regularization term which modifies the target distribution by interpolating between the temperature-scaled teacher distribution and the soft-labels of the initial parameters of the student. This corresponds to using both $\theta^{\text{\tiny teacher}}_{\{L, H\} - i}$ and $\theta^{\text{\tiny teacher}}_{i}$ as teachers, when distilling to $\theta^{\text{\tiny student}}_{i}, \, i \in \{L, H\}$. The former teacher is used to predict soft-labels for distillation, while the latter  acts as a regularizer, preventing the student model from drifting too far from the parameters at the start of the distillation round.


We use the Kullback–Leibler divergence~\citep{murphy2022probabilistic} between the student probabilities and the target probabilities as the distillation loss. For both \merged\ and \inter, we optimize the distillation updates with Adam using the default hyper-parameters. For each student optimizer, we tune a learning rate that decays linearly over the course of all federated rounds.

Though either method can be trivially extended to incorporate labeled distillation data by tuning an additional interpolating value between the teacher soft-labels and the true one-hot labels, in all experiments, we use only unlabeled distillation data. Our goal is to avoid any gains by exposing the models to additional labeled data and, thus, demonstrate the improvements solely due to codistillation. Nonetheless, unlabeled data is easier to acquire in practice than labeled data, especially in our domain of interest.
 
% \subsubsection{\inter}
In all experiments with \inter, we set the codistillation period to $p=200$ rounds and run codistillation for $s=200$ steps each codistillation round. When running \inter, we reset the momentum variables of the \fedavg\ optimizers after each codistillation round, as the models have departed from their initial parameters, rendering the momentum stale. When running \merged, we take $s=32$ distillation steps to form each round's distillation gradient. %When combining the \fedavg\ and distillation gradients in \merged, we re-scale the norm of the merged gradient to the size of the original \fedavg\ gradient. 

